EXIT: Context-Aware Extractive Compression for Enhancing Retrieval-Augmented Generation

We introduce EXIT, an extractive context compression framework that enhances both the effectiveness and efficiency of retrieval-augmented generation (RAG) in question answering (QA). Current RAG systems often struggle when retrieval models fail to rank the most relevant documents, leading to the inclusion of more context at the expense of latency and accuracy. While abstractive compression methods can drastically reduce token counts, their token-by-token generation process significantly increases end-to-end latency. Conversely, existing extractive methods reduce latency but rely on independent, non-adaptive sentence selection, failing to fully utilize contextual information. EXIT addresses these limitations by classifying sentences from retrieved documents - while preserving their contextual dependencies - enabling parallelizable, context-aware extraction that adapts to query complexity and retrieval quality. Our evaluations on both single-hop and multi-hop QA tasks show that EXIT consistently surpasses existing compression methods and even uncompressed baselines in QA accuracy, while also delivering substantial reductions in inference time and token count. By improving both effectiveness and efficiency, EXIT provides a promising direction for developing scalable, high-quality QA solutions in RAG pipelines. Our code is available at https://github.com/ThisIsHwang/EXIT

==> fig/Figure3.tex <==
\begin{figure}[]
\centerline{\includegraphics[width=0.5\linewidth]{Figure5.pdf}}
    \caption{Overview of our framework. First, the retrieved document is split into sentences. Next, each sentence is evaluated as either ``Yes" or ``No" using the Compressor. Finally, sentences with scores above the threshold are recombined in their original order to complete the compression.} \label{fig:fig5}
\end{figure}

==> fig/Figure5.tex <==
\begin{figure*}[]
\centerline{\includegraphics[width=\linewidth]{Figure10.pdf}}
    \caption{Performance analysis across different top-k values (1, 5, 10, 20, 30). Upper: Comparison of performance and token retention between baselines and our method. Lower: Compression, reading, and total inference times. Experiments were conducted on a single A100-80GB GPU.} \label{fig:trend_latency}
\end{figure*}

==> fig/Figure6.tex <==
\begin{figure*}[]
\centerline{\includegraphics[width=\linewidth]{Figure7.pdf}}
    \caption{Overview of our framework. First, the retrieved document is split into sentences. Next, each sentence is evaluated as either ``Yes" or ``No" using the Compressor. Finally, sentences with scores above the threshold are recombined in their original order to complete the compression.} \label{fig:fig6}
\end{figure*}

==> fig/Figure7.tex <==
\begin{figure*}[]
\centerline{\includegraphics[width=\linewidth]{Figure8.pdf}}
    \caption{Overview of our framework. First, the retrieved document is split into sentences. Next, each sentence is evaluated as either ``Yes" or ``No" using the Compressor. Finally, sentences with scores above the threshold are recombined in their original order to complete the compression.} \label{fig:fig7}
\end{figure*}

==> fig/distribution.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/word_count.pdf}
    \caption{\small (Left) Distribution of token counts in \textit{DSLR}-refined documents on the NQ dataset. (Right) Comparison of \textit{DSLR} with document truncated to an average fixed length (P), document processed using sentence-level re-ranking to include only the most relevant sentences up to the average length (S), and document using random selection of sentences up to the average length (R).}
    \label{fig:distribution}
    \vspace{-0.15in}
\end{figure}


==> fig/dslr.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{fig/fig2.pdf}
    \caption{
\small Comparison of the conventional RAG pipeline (top) and our sentence-level re-ranking and reconstruction framework (bottom) in an RAG system. Initially, both methods retrieve query-relevant documents at the passage level. The conventional approach directly utilizes these passages, which may contain redundant information leading to QA inaccuracies. By contrast, our method decomposes passages into sentences, re-ranks them based on relevance, and reconstructs them into coherent passages for more accurate LLM responses.}
    \label{fig:dslr}
    \vspace{-0.125in}
\end{figure*}

==> fig/effectiveness.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/ef.pdf}
    %\caption{Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and passage-level across various open-domain QA datasets.}
    \caption{\small Comparative average performance of sentence-level and passage-level re-ranking across the dataset with a context length of 100 words.}
% Comparison of passage-level and sentence-level reranking accuracy (acc) on the NQ dataset. The left graph shows accuracy improvements with increasing context length (\(L\)), and the right graph shows accuracy improvements with increasing initial retrieval depth (\(N\)).}
    \label{fig:effective}
    \vspace{-0.15in}
\end{figure}


==> fig/model_comparision.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/model_comparison.pdf}
    \caption{
    Distribution of relevance scores for 1,000 randomly sampled documents from the NQ, TQA, and SQD datasets for each model.
    }
    \label{fig:model_comparison}
\end{figure*}

==> fig/motivation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/model_comparison.pdf}
    \caption{
    Distribution of relevance scores for 1000 randomly sampled documents from the NQ, TQA, and SQD datasets for each model.
    }
    \label{fig:model_comparison}
\end{figure}

==> fig/oracle.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/threshold_vs_acc_tokens.pdf}
    %\caption{Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and passage-level across various open-domain QA datasets.}
    \caption{\small 
Variation in accuracy and token count (\# tok) with adjustments to threshold 
\(T\) on the SQD dataset, with dashed lines indicating oracle accuracy and corresponding token count.}
% Comparison of passage-level and sentence-level reranking accuracy (acc) on the NQ dataset. The left graph shows accuracy improvements with increasing context length (\(L\)), and the right graph shows accuracy improvements with increasing initial retrieval depth (\(N\)).}
    \label{fig:oracle}
    \vspace{-0.15in}
\end{figure}


==> fig/precision.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/precision.pdf}
    %\caption{Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and passage-level across various open-domain QA datasets.}
    \caption{\small Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and the passage-level baseline (Passage).}
% Comparison of passage-level and sentence-level reranking accuracy (acc) on the NQ dataset. The left graph shows accuracy improvements with increasing context length (\(L\)), and the right graph shows accuracy improvements with increasing initial retrieval depth (\(N\)).}
    \label{fig:precision}
    \vspace{-0.15in}
\end{figure}


==> fig/recomp.tex <==
\begin{figure*}

    \centering
    
    \includegraphics[width=1\linewidth]{fig/rc.pdf}
    %\caption{Performance comparison of \textit{DSLR} and RECOMP \cite{recomp} across multiple open-domain QA datasets with models including Contriever, RankT5, and RG for \textit{DSLR}, and extractive (Extr.) and abstractive (Abst.) models for RECOMP. The in-domain (Hatched) results refer to models trained specifically for the dataset.}
    
    % \vspace{-0.15in}
        \caption{\small Performance comparison of \textit{DSLR} and RECOMP \cite{recomp} across multiple open-domain QA datasets, featuring models including Contriever, RankT5, and RG for \textit{DSLR}, and extractive (Extr.) and abstractive (Abst.) models for RECOMP. The in-domain (Hatched) results refer to models specifically trained for the dataset.}
    \label{fig:recomp}
\end{figure*}

==> fig/robustness.tex <==
\begin{figure}[t!]
    \vspace{-0.07in}
    \centering
    \includegraphics[width=1\linewidth]{fig/reranking_strategies_comparison_combined.pdf}
    \caption{\small Comparison of the passage-level baseline and \textit{DSLR} with sentence-level re-ranking by varying context lengths (\(L\)) and initial retrieval depths (\(N\)) on the NQ dataset. %The left graph shows accuracy across varying context lengths (\(L\)), and the right graph details accuracy across different initial retrieval depths (\(N\)).
    }
    \label{fig:robustness}
    \vspace{-0.15in}
\end{figure}

==> fig/various.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{fig/vr.pdf}
    %\caption{Golden Answer Hit Rate after re-ranking for top-100 retrieved documents, comparing \textit{DSLR} (Sentence) and passage-level across various open-domain QA datasets.}
    \caption{\small Comparison between the Baseline (original  documents) and Ours (\textit{DSLR}-refined documents using MonoT5) in the top-\(N\) multiple passages scenario on the NQ dataset. (Left) Accuracy (Acc) as top-\(N\) increases. (Center) Average token count (\# tok) as top-\(N\) increases. (Right) Average end-to-end latency (E2E) as top-\(N\) increases, measured in seconds.}
% Comparison of passage-level and sentence-level reranking accuracy (acc) on the NQ dataset. The left graph shows accuracy improvements with increasing context length (\(L\)), and the right graph shows accuracy improvements with increasing initial retrieval depth (\(N\)).}
    \label{fig:various}
    \vspace{-0.15in}
\end{figure*}


==> table/classifier.tex <==
% \begin{table}[ht]
%     \centering
%     \caption{Classification performance for Yes/No labels with overall accuracy.}
%     \label{tab:table5.2}
%     \small
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{>{\centering\arraybackslash}p{3cm}|>{\centering\arraybackslash}p{3cm}|>{\centering\arraybackslash}p{3cm}|>{\centering\arraybackslash}p{3cm}}
%  \multicolumn{4}{c}{\textbf{Overall}}\\
%         \toprule
%         \textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\ 
%         \midrule
%         Yes & 0.91 & 0.93 & 0.92 \\ 
%         No & 0.93 & 0.91 & 0.92 \\
%         \midrule
%  \multicolumn{4}{c}{\textbf{Hard Negative}}\\
%  \midrule
%  \textbf{Class} & \textbf{Precision} & \textbf{Recall} &\textbf{F1-Score} 
% \\
% \midrule
%  Yes & 0.86& 0.93 &0.89\\
%  No & 0.93 & 0.84&0.88\\
%  \midrule
%  \multicolumn{4}{c}{\textbf{Negative}}\\
%  \midrule
%  \textbf{Class} & \textbf{Precision} & \textbf{Recall} &\textbf{F1-Score} 
% \\
%  \midrule
% Yes & 0.96& 0.93 &0.95\\
% No & 0.93& 0.96&0.95\\
% \midrule
%     \end{tabular}
%     }
%     \vspace{0.5em}\\
%     % \textit{Accuracy: 0.92}
% \end{table}

\begin{table}[]
    \centering
    \small
    \caption{Classification performance for Yes/No labels with overall accuracy.}
    \label{tab:table5.2}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{c|c|c|c}
        \multicolumn{4}{c}{\textbf{Overall}} \\
        \toprule
        \textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\ 
        \midrule
        Yes & 0.91 & 0.93 & 0.92 \\ 
        No & 0.93 & 0.91 & 0.92 \\
        \midrule
        \multicolumn{4}{c}{\textbf{Hard Negative}} \\
        \midrule
        Yes & 0.86 & 0.93 & 0.89 \\
        No & 0.93 & 0.84 & 0.88 \\
        \midrule
        \multicolumn{4}{c}{\textbf{Negative}} \\
        \midrule
        Yes & 0.96 & 0.93 & 0.95 \\
        No & 0.93 & 0.96 & 0.95 \\
        \bottomrule
    \end{tabular}
\end{table}

==> table/simple_sparse.tex <==
\begin{table}[]
    \centering
    \small
    \caption{Performance comparison using BM25. Best results are highlighted in \textbf{bold}.}
    \label{tab:simple_sparse_retrieval}
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.1}
    \small
    \begin{tabular}{l|cc}
        \toprule[1.5pt]
        \textbf{Compressor} & \scriptsize EM $\uparrow$ & \scriptsize F1 $\uparrow$ \\
        \midrule[1pt]
        Original Docs   & 28.2 & 39.1 \\
        \midrule[0.8pt]
        RECOMP-Extr    & 28.2 & 37.5 \\
        RECOMP-Abst    & 27.8 & 39.2 \\
        LongLLMLingua  & 28.6 & 39.7 \\
        CompAct        & 30.6 & 41.2 \\
        \rowcolor{blue!5} EXIT (Ours)  & \textbf{33.4} & \textbf{44.5} \\
        \bottomrule[1.5pt]
    \end{tabular}
\end{table}
